Hierarchical Mixture of Experts: Generalizable Learning for High-Level Synthesis

High-level synthesis (HLS) is a widely used tool in designing Field Programmable Gate Array (FPGA). HLS enables FPGA design with software programming languages by compiling the source code into an FPGA circuit. The source code includes a program (called "kernel") and several pragmas that instruct hardware synthesis, such as parallelization, pipeline, etc. While it is relatively easy for software developers to design the program, it heavily relies on hardware knowledge to design the pragmas, posing a big challenge for software developers. Recently, different machine learning algorithms, such as GNNs, have been proposed to automate the pragma design via performance prediction. However, when applying the trained model on new kernels, the significant domain shift often leads to unsatisfactory performance. We propose a more domain-generalizable model structure: a two-level hierarchical Mixture of Experts (MoE), that can be flexibly adapted to any GNN model. Different expert networks can learn to deal with different regions in the representation space, and they can utilize similar patterns between the old kernels and new kernels. In the low-level MoE, we apply MoE on three natural granularities of a program: node, basic block, and graph. The high-level MoE learns to aggregate the three granularities for the final decision. To train the hierarchical MoE stably, we further propose a two-stage training method to avoid expert polarization. Extensive experiments verify the effectiveness of the proposed hierarchical MoE. We publicized our codes at https://github.com/weikai-li/HierarchicalMoE.

==> 7.checklist.tex <==
\section{Reproducibility Checklist}

This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. (yes/partial/no/NA) Yes.
    \item Clearly delineates statements that are opinions, hypotheses, and speculations from objective facts and results. (yes/no) Yes.
    \item Provides well-marked pedagogical references for less-familiar readers to gain the background necessary to replicate the paper. (yes/no) Yes.
\end{itemize}

\noindent Does this paper make theoretical contributions? (yes/no) No.
\noindent If yes, please complete the list below.
\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
\item Proofs of all novel claims are included. (yes/partial/no)
\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
\item Appropriate citations to theoretical tools used are given. (yes/partial/no)
\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
\item All experimental codes used to eliminate or disprove claims are included. (yes/no/NA)
\end{itemize}

\noindent Does this paper rely on one or more datasets? (yes/no) Yes.
\noindent If yes, please complete the list below.
\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets. (yes/partial/no/NA) Yes.
\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) NA (We only used existing public benchmark datasets).
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) NA (We only used existing public benchmark datasets).
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) Yes.
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) Yes.
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying. (yes/partial/no/NA) NA (We only used public benchmark datasets).
\end{itemize}

\noindent Does this paper include computational experiments? (yes/no) Yes.
\noindent If yes, please complete the list below.
\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. (yes/partial/no) Yes.
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) Yes.
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) Yes.
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. (yes/partial/no) Yes.
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) Yes.
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names, and versions of relevant software libraries and frameworks. (yes/partial/no) Yes.
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) Yes.
\item This paper states the number of algorithm runs used to compute each reported result. (yes/no) Yes.
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) Yes.
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) Partial (We run the offline evaluation experiments five times and online evaluation experiments three times, and we report the mean performance and the standard deviation).
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) Yes (The most important hyper-parameters are listed in the appendix. Others are in the codes that we submit).
\item This paper states the number and range of values tried per (hyper-) parameter during the development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) Yes.
\end{itemize}
